Minimization of Visibly Pushdown Automata Using Partial Max-SAT

We consider the problem of state-space reduction for nondeterministic weakly-hierarchical visibly pushdown automata (VPA). VPA recognize a robust and algorithmically tractable fragment of context-free languages that is natural for modeling programs. We define an equivalence relation that is sufficient for language-preserving quotienting of VPA. Our definition allows to merge states that have different behavior, as long as they show the same behavior for reachable equivalent stacks. We encode the existence of such a relation as a Boolean partial maximum satisfiability (PMax-SAT) problem and present an algorithm that quickly finds satisfying assignments. These assignments are sub-optimal solutions to the PMax-SAT problem but can still lead to a significant reduction of states. We integrated our method in the automata-based software verifier Ultimate Automizer and show performance improvements on benchmarks from the software verification competition SV-COMP.

==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

To the best of our knowledge, we are the first to address the minimization problem for the general class of weakly-hierarchical \vpa and \bvpa.
For this purpose, we synthesized an equivalence relation from a \pmaxsat instance.
The \pmaxsat constraints ensure that the minimization is language-preserving and that unreachable configurations do not prevent the merging of states.

\smallskip

A possible line of future work is to extend our ideas to other minimization approaches 
(e.g., Hopcroft's algorithm~\cite{Hopcroft:1971} or simulation-based algorithms~\cite{EtessamiEtal:2005}).

\TodoCM{Remove the conclusion?}

